A Survey on Visualization Approaches in Political Science for Social and Political Factors: Progress to Date and Future Opportunities

Politics is the set of activities related to strategic decision-making in groups. Political scientists study the strategic interactions between states, institutions, politicians, and citizens; they seek to understand the causes and consequences of those decisions and interactions. While some decisions might alleviate social problems, others might lead to disasters such as war and conflict. Data visualization approaches have the potential to assist political scientists in their studies by providing visual contexts. However, political researchers' perspectives on data visualization are unclear. This paper examines political scientists' perspectives on visualization and how they apply data visualization in their research. We discovered a growing trend in the use of graphs in political science journals. However, we also found a knowledge gap between the political science and visualization domains, such as effective visualization techniques for tasks and the use of color studied by visualization researchers. To reduce this gap, we survey visualization techniques applicable to the political scientists' research and report the visual analytics systems implemented for and evaluated by political scientists. At the end of this paper, we present an outline of future opportunities, including research topics and methodologies, for multidisciplinary research in political science and data analytics. Through this paper, we expect visualization researchers to get a better grasp of the political science domain, as well as broaden the possibility of future visualization approaches from a multidisciplinary perspective.

==> 0_bio.tex <==
\section*{Short Biographies of Authors}
 
\subsection*{Dongyun Han} 
Dongyun Han is a Ph.D. student in the department of Computer Science at Utah State University. His research interests include visual analytics, data visualization, and human-computer interaction. He has been developing visual analytics systems for several research domains including Earth Science, Political Science, History, and Distributed Energy resources. 
He received a M.S in Computer Science at Ulsan National Institute of Science and Technology (UNIST) in 2020.   

\subsection*{Abdullah-Al-Raihan Nayeem} 
Abdullah-Al-Raihan Nayeem is a Ph.D. student in Computer Science at the University of North Carolina at Charlotte. He has extensive experience working in the enterprise application platforms, followed by pursuing a career in research. His research interests are visual analytics systems, interactive geo-spatiotemporal visualization, and distributed data analysis. 

\subsection*{Jason Windett}
Jason Windett is an Associate Professor of Political Science and Public Administration, Associate Professor of Public Policy, and a Faculty Affiliate in the School of Data Science at the University of North Carolina at Charlotte. His main research interests are political representation, state politics, and political methodology. He has served as a principal investigator on multiple projects sponsored by the National Science Foundation including “Building the Federalism Data and Advanced Statistics Hub” and “ the Institutional Foundations of Judicial Independence”.  He is currently a co-PI on “Systematic Content Analysis of Litigation EventS Open Knowledge Network” funded by the NSF’s Convergence Accelerator. He was previously a co-PI on “Diffusion Analytics for Public Policy Research.” He received his Ph.D. in Political Science from the University of North Carolina at Chapel Hill. 

\subsection*{Yaoyao Dai}
Yaoyao Dai is an assistant professor in the Department of Political Science and Public Administration at the University of North Carolina at Charlotte. She received a dual-title Ph.D. in Political Science and Asian Studies from the Pennsylvania State University. Her research focuses on information manipulation, populism, authoritarian politics, and text as data. 

\subsection*{Ben Radford}
Ben Radford is an assistant professor of Political Science and Public Administration, a faculty member of the Public Policy Ph.D. Program, an affiliate member of the School of Data Science, and a member of the CyberDNA Center at UNC Charlotte. His research focuses on political methodology and applications of machine learning to political conflict, cybersecurity, and international relations. He is particularly interested in extracting structured information about political and cybersecurity-relevant events from unstructured text data.

\subsection*{Isaac Cho}
Isaac Cho received his Ph.D. in Computing and Information Systems from the University of North Carolina at Charlotte in 2013. He is an assistant professor in the Computer Science department at Utah State University and an adjunct professor in the Computer Science department at the University of North Carolina at Charlotte. He is also a faculty member of the Ribarsky Center for Visual Analytics at the University of North Carolina at Charlotte and he directs the VizUS lab (Visualization lab at Utah State) at Utah State University. His main research interests are interactive visual analytics, data visualization, and human-computer interactions. He is senior personnel of the NSF Data  Infrastructure  Building  Blocks project and a co-principal investigator of two NSF-funded projects including "Building the Federalism Data and Advanced Statistics Hub”. He was also a member of the VACCINE Center, a DHS Center of Excellence. He has been leading visual analytics research for US government-funded research projects. 


==> 6_1_discussion_perspective_in_political_science.tex <==


% \begin{figure}[hbt!]
%     \centering
%     \includegraphics[width=.4\textwidth]{overview.pdf}
%     \caption{Percentage of articles mentioning ''visualization'' or ''visualize'' or ''plot'' or ''graph'' or ''figure'', data from Constellate
%     %https://constellate.org/builder/?keyword=%22data%20visualization%22&start=1900&end=2022&category=Political%20science
%     }
%     \label{fig:overview}
% \end{figure}





  

\subsection{Knowledge Gap in Visualization}
Political scientists are becoming more familiar with visual analytics tools, specifically the increasingly common web-based dashboards associated with major data collection projects. For example, the Armed Conflict Location and Event Data Project (ACLED) maintains a dashboard for users interested in quickly assessing the scope and trends present in their data \cite{raleigh:etal:2010}. The Peace Research Institute of Oslo maintains a similar dashboard associated with their GRID dataset \cite{tollefsen:etal:2012}. The Manifesto Project provides four ``simple dashboards'' on its website and links to external researchers' dashboards based on Manifesto data \cite{merz:etal:2016}. These tools and others like them allow researchers to quickly inspect available data and assess whether they are suitable for their research purposes. 
% In that sense, dashboards associated with data collection and distribution efforts serve to market the data by demonstrating its use in simple analyses or by providing summary statistics. They can also prove useful for ``sanity checking'' data issues: researchers can quickly compare their own downloaded and munged copies of the data against the values in the dashboard. The dashboards may also be of interest to more general audiences interested in political science topics but lacking the formal analytical skills necessary to generate their own visualizations. 

As we discussed in the previous section, political scientists still used visualizations mainly to report their results to evaluate the hypothesis. However, earlier visualization researchers coordinated with political scientists showed that visualization approaches could be more beneficial to them such as the following stages~\cite{borkin2013makes}: (1) Exploring and familiarizing large data sets; (2) Identifying trends and unexpected patterns; (3) Generating hypotheses; and (4) Analyzing and verifying statistical findings. 
% (5) Picture the superiority phenomenon that makes data more memorable than expressing it in tables or words.

\subsection{Opportunity for Multidisciplinary Research}

\HDY{
Over the last few decades, government institutions and political scientists have amassed numerous types of data, including government statistics to aid in global and subnational contextual understanding. Political actors are now challenged to evaluate and analyze the situation and dynamic connections of global and subnational governments using large amounts of qualitative and quantitative information. 
% The field of data visualization has a great potential to assist policymakers and political scientists in their responsibilities by providing visualized contexts such as the following stages~\cite{borkin2013makes}: (1) Exploring and familiarizing large data sets; (2) Identifying trends and unexpected patterns; (3) Generating hypotheses; (4) Analyzing and verifying statistical findings; (5) Picture the superiority phenomenon that makes data more memorable than expressing it in tables or words.
}

% There are several avenues by which political scientists may benefit from adopting visual analytics. In this section, we highlight some opportunities for multidisciplinary research. We are particularly optimistic about the application of visual analytics to data wrangling (``munging''), dataset selection or promotion theory and hypothesis formation, communicating results or research processes with diverse audiences, and for soliciting information from research subjects (e.g. survey respondents). We also propose that visual analytics may help political scientists select better priors for their analyses while also recognizing that this practice may need to be balanced against the subjectivity (and possible loss of reproducibility) that comes with interactive user interfaces. 

% \subsubsection{Dataset selection or promotion}



% In addition to using existing data, political scientists also produce all types of data for replication and future research. Visual analytics can assist in delivering those data. Researchers can gain some knowledge of a dataset or a database before downloading and analyzing the data, which potentially increases the transparency and reproducibility of the associated projects. 

A major shortcoming of Political Scientists is translating their findings to broader audiences which is often times a result of the complexity of the studies and not appropriately visualizing results to a mass audience. Using state-of-the-art visualization techniques in both publishing and training would allow Political Scientists to make a better real-world impact. Political scientists often do not have the average reader or citizen in mind when producing scientific knowledge. As such, political science research often targets only those with advanced degrees in Political Science. 

A major area of collaboration between visualization scholars and political scientists can occur in the project planning phase. Political science can benefit by interviewing potential target audiences on how to visualize data from the research design phase. By working with back-end users during design, scholars in political science can have a broader understanding of the needs of those outside the discipline. 

% \subsubsection{As an experimental tool}

% Finally, we suspect that visual analytics may have a role to play in the solicitation of data from research subjects. Providing interactive visualization tools to survey respondents, for instance, may help researchers to provide respondents with more information than they are otherwise able to by allowing those respondents to ``drive'' their information ingestion. In other words, visual analytics may prove a more appealing information transmission method for survey respondents who need to consume a large amount of data prior to answering a questionnaire than would the equivalent amount of text or static images. The ability to track the respondent as they interact with visual analytics tools may also prove helpful for political scientists interested in the saliency of different items about which information is available through the tool.


% {\color{red} Ben's notes:
% \begin{itemize}
%     \item One theme is ``bigger data needs to be analyzed faster'' -- how does this apply to Political Science? We've seen growth in political event data and textual data. Any others?
%     \item Another theme is confirmatory data analysis $\rightarrow$ exploratory data analysis. Need to reconcile this with PS disdain for data mining.
%     \item Visual analytics seem to be most useful for complex tasks that must be performed repeatedly or continuously. These are uncommon in political \textit{science} -- we rarely perform the same analysis repeatedly.
%     \item It seems to me that there's a place for visual analytics in survey research.
% \end{itemize}
% }

%\begin{itemize}
%    \item American Politics
%    \begin{itemize}
%        \item Q1: In Federalist 78, Alexander Hamilton argues for an independent judiciary that interprets laws, rather than following public preferences and other institutions. In reality, this has been a central test in studies of judicial politics for decades. Are judges independent interpreters of law, or do they use their political ideology in decisonmaking?  
%        \item Q2: Do elected officials respond to public opinion when preparing and voting on bill proposals?
%        \item Q3: How does a candidate's race and/or gender impact running and winning public office?
%        \item Q4: Why do individuals vote in elections? 
%    \end{itemize}
%    \item International Relations
%    \begin{itemize}
%        \item International Political Economy
%        \item International Conflict
%        \begin{itemize}
%            \item Q1: There's an empirical finding that democracies rarely (never???) fight wars against one another. Why not? Leading theories include increased trade ties, normative values, transparency, and membership in shared institutions.
%            \item Q2: Why have international wars decreased in frequency over the 20th and 21st centuries while civil wars have increased in frequency? 
%            \item Q3: IR scholars are perennially interested in the causes of and predictors of international conflict.
%            \item Q4: The oldest (?) puzzle in international conflict is why countries fight wars to begin with. Shouldn't they always negotiate a settlement? Fearon (1995) addresses this in what is maybe the best article ever written in IR. But I don't think that most IR scholars consider this the final word on war.
%        \end{itemize}
%    \end{itemize}
%    \item Comparative Politics



    


%\end{itemize}

%\subsubsection{Analysis Methods used in the field of Political Science}

%{\color{red}
%\emph{Ben says:}
%\begin{itemize}
%    \item Regression / generalized linear models.
%    \item Bayesian regression modeling (which brings with it trace plots).
%    \item Political science tends to be a few years behind the state of the art in ML methods, but it would be hard to find many ML methods that haven't made their way into at least a few PS papers.
%    \begin{itemize}
%        \item LDA is still super hot.
%        \item Text analysis and NLP in general are popular.
%        \item There's less work on image or video analysis (but not none).
%    \end{itemize}
%    \item Prediction and forecasting are still somewhat marginalized in political science.
%    \item Statistical inference and causal inference are still king.
%    \item Game theory / formal models. (These are becoming less common IMO.)
 %   \item Agent based models and computational models. (Again, these are declining in popularity. I bet they'll make a comeback eventually, though.) 
%\end{itemize}}
% - 
%\subsubsection{Political Science for Public}
%- visualization approach on education purposes

%\subsection{Challenges}
% - ...


==> 6_2_discussion_vis_for_public.tex <==
% \needClarification{\subsection{Visualization Approaches for Citizen}}
% ...


\subsubsection{Increased interest and need in analyzing unstructured data}

Much like policy diffusion, protests, and civil conflicts often spread geographically. Although political scientists acknowledge such spillover effects, scholars still primarily model such events in one area as independent of events in neighboring areas due to methodological constraints. 

Given the limited and often unreliable structured data in authoritarian regimes, such as government-released statistics, comparative scholars have begun to collect and analyze rich unstructured or loosely structured datasets that comprise, for example, news articles, speeches, and social media network data. Unlike traditional tabular data, unstructured and loosely structured data are often voluminous and noisy. Visual analytics can potentially assist researchers to identify and collect the appropriate data and help them to expose patterns or puzzles that stimulate new research. Furthermore, to the extent that these data are hierarchical or network-structured, interactive graph layouts with adjustable parameters will help researchers to assess the topology of such data and make informed decisions about how best to model those data (by identifying communities that should be controlled, for instance). 

\subsubsection{Communicating with diverse audiences}

We believe that visual analytics are underutilized as a communication medium between political scientists and technical and general audiences. Innovative projects such as Distill (\url{https://www.distill.pub}), now on hiatus, have demonstrated how effectively web-based publications can use interactive visualizations to communicate complicated concepts to large audiences. Distill is a peer-reviewed, Web-first academic journal of machine learning. Articles, published primarily online, may contain full-color, animated, and interactive figures. Were similar venues available for political scientists, readers might appreciate the ability to inspect model forecasts, compare observed values to predicted values, select specific models to compare side-by-side, plot user-specified marginal effects, or recreate main-paper figures using models that were otherwise relegated to appendices, among other things. In the hands of the public, tools like these may improve political science literacy and encourage readers to expand their interest in the field. For researchers, these tools could inspire and inform follow-up studies.

In addition to solving the problem of \textit{how} publishing complex visualizations, Distill also solved a more intimidating problem faced by researchers: How to receive credit for their publications outside of the physical journal space. Despite the fact that many journals have largely moved article distribution online, they nonetheless impose on the authors' antiquated rules suited for print publication. These compromises make less and less sense as readers continue to transition to online subscription models. Political science journals may benefit from a hybrid model in which print readers are pointed to supplemental online materials (as they often already are for appendices), including visual analytics tools.

==> 6_3_discussion_concerns.tex <==
\subsection{\needClarification{Considerations}}



==> README <==
Created by Torsten Moeller (vis@cs.sfu.ca), April 6 2004
modified by Steven Bergner and Torsten Moeller, June 30 2006
modified by James Peltier and Torsten Moeller, March 28, 2007
modified by Bernhard Finkbeiner, July 5, 2010
modified by Tobias Isenberg, January 2016
modified by Filip Sadlo, March 2016
modified by Tobias Isenberg, July 2016

This distribution provides a document class for formatting papers according to the specifications for submission to conferences sponsored by the IEEE Visualization & Graphics Technical Committee (VGTC).

Conferences that use the 'journal' document option:
- IEEE Visualization Conference (VIS, incl. InfoVis, SciVis, VAST)
- IEEE Virtual Reality (VR)
- IEEE International Symposium on Mixed and Augmented Reality (ISMAR)

It contains 13 files/directories:

README          - this file
diamondrule.eps - abstract and body separator
diamondrule.pdf - its PDF version
vgtc.cls        - the VGTC class file, which should be placed, somewhere in the TeX search path (or in the local directory)
template.tex    - an example paper
template.bib    - a small bibliography file used by the example
template.pdf    - an example proper pdf output in default journal mode
abbrv-doi*.bst  - four different versions to generate the bibliography including DOI output, with and without hyperref support, with and without narrow rendering of DOIs
makefile        - makefile including bibtex compilation and proper PDF generation
pictures/       - subdirectory with sample images, both in EPS and in direct pixel/vector format

Usage
=====

The template can be used as such (using the established LaTeX environments) by calling pdfLaTeX or LaTex. For Windows-based LaTeX installations you can use, for example, the environment provided by http://www.texniccenter.org/ along with MikTeX (http://miktex.org/). For Uinux-based installations, please use your favorite LaTeX distribution and editing environment or use the makefile following the instructions below.

Use of the Makefile
===================

Prior to "building" a paper please be sure to run

  make clean

This will ensure that the paper is built cleanly each and every time. We suggest to run this command before each new compilation.

To compile the example, run

  make

or manually, if the makefile does not work for you

  latex template
  bibtex template
  latex template
  latex template

If you run 'make' for the first time, a successful compilation will create a file called 'template.pdf'. Please make sure, that its layout is identical to the file 'template-journal.pdf' provided with this package.

The included makefile also allows you to run each step of the process manually.  Below are a list of available options that may be passed to make

 "make clean"
   removes all files that can be generated automatically.

 "make gs7"
   This will perform all functions to build a proper paper using GhostScript 7.

 "make gs8"
   This will perform all functions to build a proper paper using GhostScript 8.

 "make dvi"
   This will process the .tex file and produce a DVI output file.  This
   step may process the .tex file several times to process all references
   and citations.

 "make ps"
   This will process the .tex file and the DVI output and convert it to a
   PostScript file.

 "make pdf"
   This will process the .tex file using pdfTeX/pdflatex to produce a PDF
   file directly (not using a DVI and PostScript file).
   Please make sure that all fonts are embedded.
   You can use pdffonts my_document.pdf to check if they are.
   It is standard in all modern latex distributions.
   If you use eps figures (e.g. R or gnuplot figures) which you convert to
   PDF using epstopdf, do the following:
   Use GL_OPTIONS, a global environment variable for ghostscript:
   export GS_OPTIONS="-dEmbedAllFonts=true -dPDFSETTINGS=/printer"
   # and run
   epstopdf myfile.eps

   See http://bugs.debian.org/cgi-bin/bugreport.cgi?bug=411651 for the
   origin of this solution.


If you have problems with the makefile please notify us with the output of
the errors produced when running make and we will work to figure out the
resolution.


To produce proper pdf output, please use:
  dvips -t letter -Pdownload35 -Ppdf -G0 template.dvi -o template.ps

The "-Ppdf" and "-G0" flags should be specified in that order; reversing
them does not work, and will result in unacceptable results.

The following information is an exerpt from the ACM SIGGRAPH Conference /
Symposium / Workshop Content Formatting Instructions which can be found
here.

 http://www.siggraph.org/publications/instructions/author-instructions.pdf

If you are using version 7.x of GhostScript, please use the following
method of invoking ‘ps2pdf,’ in order to embed all typefaces and ensure
that images are not downsampled or subsampled in the PDF creation process:

 ps2pdf -dCompatibilityLevel=1.3 -dMaxSubsetPct=100 \
        -dSubsetFonts=true -dEmbedAllFonts=true \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

If you are using version 8.x of GhostScript, please use this method in
place of the example above:

 ps2pdf -dPDFSETTINGS=/prepress -dCompatibilityLevel=1.3 \
        -dAutoFilterColorImages=false -dAutoFilterGrayImages=false \
        -dColorImageFilter=/FlateEncode -dGrayImageFilter=/FlateEncode \
        -dMonoImageFilter=/FlateEncode template.ps template.pdf

This has been incorporated into the makefile and should no longer be needed
unless you are building the PDF file manually.


==> makefile <==
# This file seems to originate from something called 'the ultimate
# latex makefile' that different authors worked on. Find original
# versions at:
# http://tadek.pietraszek.org/blog/2006/03/24/the-ultimate-latex-makefile/
# (c) by Tadeusz Pietraszek
# http://www.acoustics.hut.fi/u/mairas/UltimateLatexMakefile/ 
# (c) by Matti Airas
#
# This file has been assembled and adjusted by Steven Bergner, Nov 2005
#  - support for multiple sub-texfiles
#  - fixed '=' '#' problem in mingw/msys environment (see E variable)
#  - PS compilation uses VGTC recommended settings
#  - targets restructured to make PDF by default
#
# Call 'make dvi' for minimal compilation, to check for proper latex
# syntax. This can be much faster than a full PDF generation when big
# figures are involved.
#
# Call 'make pdf' for direct compilation to PDF using pdfTeX. Note that this
# requires you to use .pdf files. pdfTeX can not use .ps or .eps graphics.
# use epstopdf to convert such files to .pdf files.
#
#----------------------------------------------------------------------------
#adjust the following for your purpose

#set the a .dvi name that corresponds to your main .tex file
DVIFILES = template.dvi
MAINTEXFILE = $(DVIFILES:.dvi=.tex)
SUBTEXFILES = 
BIBFILES = template.bib

#switch = to # when using ps2pdf in win32 (mingw/msys), i.e. uncomment 2nd line
#E=\=
E=\#

#adjust paper size: letter/a4
PAPERSIZE=letter
PDFLATEXPAPERSIZE="-sPAPERSIZE$E$(PAPERSIZE)"
DVIPSPAPERSIZE=-t $(PAPERSIZE)
#uncomment the following two lines when using option tvcgpapersize
#DVIPSPAPERSIZE=-T 7.875in,10.75in
#PDFLATEXPAPERSIZE=

#----------------------------------------------------------------------------
LATEX = latex
BIBTEX = bibtex
L2H = latex2html
PDFLATEX = ps2pdf
PDFTEX = pdflatex
DVIPS = dvips 

RERUN = "(There were undefined references|Rerun to get (cross-references|the bars) right)"
RERUNBIB = "No file.*\.bbl|Citation.*undefined" 

PSFILES  = $(DVIFILES:.dvi=.ps) 

PDFFILES7 = $(DVIFILES:.dvi=.pdf7) 
PDFFILES8 = $(DVIFILES:.dvi=.pdf8) 

PDFTEXFILES = $(DVIFILES:.dvi=.pdftex)

COPY = if test -r $*.toc; then cp $*.toc $*.toc.bak; fi 
#RM = /usr/bin/rm -f 
RM = rm -f 

all:	msg gs8

msg:
	@echo "  This script defaults to GhostScript 8.  If you are using GhostScipt 7 please type"
	@echo "  make gs7 instead.  If unsure type gs -v from the command line"
	@echo "  To use pdflatex/pdftex, type make pdf"
	@echo ""


pdf:     clean pdftex 

gs7:        clean dvi ps pdf7

gs8:        clean dvi ps pdf8

dvi:           $(DVIFILES)

ps:           $(PSFILES)

pdf7:           $(PDFFILES7)

pdf8:           $(PDFFILES8)

pdftex:         $(PDFTEXFILES)

$(MAINTEXFILE) : $(SUBTEXFILES) $(BIBFILES)

%.dvi:			%.tex
				$(COPY);$(LATEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(LATEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(LATEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.pdftex:			%.tex
				echo "wir sind da"
				$(COPY);$(PDFTEX) $<
				egrep -c $(RERUNBIB) $*.log && ($(BIBTEX) $*;$(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				egrep $(RERUN) $*.log && ($(COPY);$(PDFTEX) $<) ; true
				if cmp -s $*.toc $*.toc.bak; then . ;else $(PDFTEX) $< ; fi
				$(RM) $*.toc.bak
# Display relevant warnings
				egrep -i "(Reference|Citation).*undefined" $*.log ; true

%.ps:			%.dvi
#				dvips -T 7.875in,10.75in -Ppdf -G0 $< -o $@  #use tvcgpapersize
#				dvips -Ppdf -G0 $< -o $@
				dvips $(DVIPSPAPERSIZE) -Pdownload35 -Ppdf -G0 $< -o $@
#				dvips $< -o $@


%.pdf7:			%.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dMaxSubsetPct$E100" \
	"-dCompatibilityLevel$E1.3" \
	"-dSubsetFonts$Etrue" \
	"-dEmbedAllFonts$Etrue" \
	"-dAutoFilterColorImages$Efalse" \
	"-dAutoFilterGrayImages$Efalse" \
	"-dColorImageFilter$E/FlateEncode" \
	"-dGrayImageFilter$E/FlateEncode" \
	"-dMonoImageFilter$E/FlateEncode" \
	$< template.pdf

#				$(PDFLATEX) $<

%.pdf8:                 %.ps
	$(PDFLATEX) \
	$(PDFLATEXPAPERSIZE) \
	"-dPDFSETTINGS=/prepress" \
	"-dCompatibilityLevel=1.3" \
	"-dAutoFilterColorImages=false" \
	"-dAutoFilterGrayImages=false" \
	"-dColorImageFilter=/FlateEncode" \
	"-dGrayImageFilter=/FlateEncode" \
	"-dMonoImageFilter=/FlateEncode" \
	"-dDownsampleGrayImages=false" \
	"-dDownsampleColorImages=false" \
	$< template.pdf
#                               $(PDFLATEX) $<

# cleans anything that can be re-generated automatically, plus emacs backups
clean: 
				rm -f *.aux *.log *.bbl *.blg *.brf *.cb *.ind *.idx *.ilg	\
				*.inx *.toc *.out $(DVIFILES) $(PSFILES) template.pdf *~

.PHONY : all pdf ps dvi clean $(MAINTEXFILE)

